Ultrametric Fitting by Gradient Descent

We study the problem of fitting an ultrametric distance to a dissimilarity graph in the context of hierarchical cluster analysis. Standard hierarchical clustering methods are specified procedurally, rather than in terms of the cost function to be optimized. We aim to overcome this limitation by presenting a general optimization framework for ultrametric fitting. Our approach consists of modeling the latter as a constrained optimization problem over the continuous space of ultrametrics. So doing, we can leverage the simple, yet effective, idea of replacing the ultrametric constraint with a min-max operation injected directly into the cost function. The proposed reformulation leads to an unconstrained optimization problem that can be efficiently solved by gradient descent methods. The flexibility of our framework allows us to investigate several cost functions, following the classic paradigm of combining a data fidelity term with a regularization. While we provide no theoretical guarantee to find the global optimum, the numerical results obtained over a number of synthetic and real datasets demonstrate the good performance of our approach with respect to state-of-the-art agglomerative algorithms. This makes us believe that the proposed framework sheds new light on the way to design a new generation of hierarchical clustering methods. Our code is made publicly available at \url{https://github.com/PerretB/ultrametric-fitting}.

==> preliminaries.tex <==
%Ultrametric and hierarchical clustering

%Special case of the subdominant ultrametric (SUM) (bad acronym is bad)

Let $\G=(\V, \E)$ be an undirected graph with $\V$ a finite set of vertices and $\E$ a set of (unordered) pairs of distinct vertices representing edges. 
The edges of $\G$ are weighted by a positive function $\w\in\weightfuns={\RR_+}^{\E}$ presenting a dissimilarity measure between the vertices of $\G$. 

A \emph{partition} $P$ of $\G$ is a set of subsets of $\V$ such that $\bigcup P=\V$, any two elements of $P$ are disjoint, and any element of $P$ is connected for $\G$. 
The set of partitions of $\G$ is denoted by $\Pi_\G$.
Being given two partitions $P_1$ and $P_2$ of $\G$, we say that $P_1$ is smaller than $P_2$ if any element of $P_1$ is contained in an element of $P_2$.
A \emph{hierarchical clustering} of $\G$ is a non decreasing function $\HH$ from $\RR_+$ to $\Pi_\G$ such that  $\HH(\lambda) = \set{\V}$ for a sufficiently large value $\lambda$. 
A hierarchical clustering is often represented as a dendrogram, \ie{} as the rooted tree induced by the inclusion relation among the regions of its partitions.

Hierarchical clusterings and ultrametric distances are dual representations:
\begin{itemize}
    \item A hierarchical clustering $\HH$ induces an ultrametric distance $d_\HH$ defined by: 
\begin{equation}
\forall (x,y) \in V^2, \ d_\HH(x,y) = \min\{\lambda \mid \exists X \in \HH(\lambda), \{x,y\}\subseteq X\}
\end{equation}
    i.e. the smallest level $\lambda$ such that $x$ and $y$ belong to a same region in $\HH(\lambda)$.
    \item An ultrametric distance $d$ induces a hierarchical clustering $\HH_d$ where, for any level $\lambda$, $\HH_d(\lambda)$ is composed of the maximal regions such that there exists a path composed of edges of value lower than or equal to $\lambda$ between any two vertices.  
\end{itemize}

One classical approach to obtain an ultrametric distance from a given dissimilarity $\w$  is the \emph{subdominant ultrametric} (also known as the \emph{ultrametric opening}), \ie{} the largest ultrametric smaller than $\w$:
\begin{equation}
   \subum{\w} =  \max \set{ u \in \weightfuns \mid u \leq w \textrm{ and $u$ is an ultrametric}} 
\end{equation}
where we consider the point-wise (marginal)  ordering on functions. 
The subdominant ultrametric is strongly linked to the $\min\max$-distance, denoted by $\minmax_\G$, by the following relation: 
\begin{equation}
\forall \set{x,y}\in E, \subum{w}(\set{x,y}) = \minmax_\G(x, y).
\end{equation}
with:
\begin{equation}
\minmax_\G(x,y) = \min_{P\in \Paths_{xy}} \max_{e \in P} \w(e),
\end{equation}
where $\Paths_{xy}$ denotes the set of all paths from $x$ to $y$ in $\G$.

The hierarchical clustering corresponding to the subdominant ultrametric is known as \emph{single/min linkage clustering} which can be computed in time $\mathcal{O}(|\E|\log(|\E|))$  with a variant of Kruskal's minimum spanning tree algorithms\Cite{Gower1969}. 
On the other hand, the ultrametric $d$ corresponding to the hierarchical clustering $\HH$ can be computed in time $\mathcal{O}(|\E| + |\V|)$ thanks to a fast lowest common ancestor algorithm\Cite{Bender2000}.
The subdominant ultrametric can thus  be computed in time $\mathcal{O}(|\E|\log(|\E|))$. 

Despite its sounded definition and the existence of efficient algorithms to compute it,  the subdominant ultrametric is rarely used in practice due to its sensitivity to noise and to the \emph{leakage/chaining} problem.

